Personalized Federated Learning through Local Memorization

Federated learning allows clients to collaboratively learn statistical models while keeping their data local. Federated learning was originally used to train a unique global model to be served to all clients, but this approach might be sub-optimal when clients' local data distributions are heterogeneous. In order to tackle this limitation, recent personalized federated learning methods train a separate model for each client while still leveraging the knowledge available at other clients. In this work, we exploit the ability of deep neural networks to extract high quality vectorial representations (embeddings) from non-tabular data, e.g., images and text, to propose a personalization mechanism based on local memorization. Personalization is obtained by interpolating a collectively trained global model with a local $k$-nearest neighbors (kNN) model based on the shared representation provided by the global model. We provide generalization bounds for the proposed approach in the case of binary classification, and we show on a suite of federated datasets that this approach achieves significantly higher accuracy and fairness than state-of-the-art methods.

==> related_1.tex <==
We discuss personalized FL approaches to address statistical heterogeneity and system heterogeneity.

\subsection{Statistical Heterogeneity}
This body of work considers that all clients have the same model architecture but potentially different parameters.

A simple approach for FL personalization is learning first a global model and then fine-tuning its parameters at each client through stochastic gradient descent for a few epochs~\citep{jiang2019improving, yu2020salvaging}; we refer later to this approach as \FedAvg+. \FedAvg+ was later explained by \citet{chen2022on} and \citet{cheng2021fine}. The global model can then be considered as a meta-model to be used as initialization for a few-shot adaptation at each client. Later work~\citep{khodak2019adaptive, fallah2020personalized, emre2021debiasing} has formally established the connection with Model Agnostic Meta Learning (MAML)~\citep{jiang2019improving} and proposed different algorithms to train a more suitable meta-model for local personalization.

\texttt{ClusteredFL}~\citep{sattler2020clustered, ghosh2020efficient, mansour2020three} assumes that clients can be partitioned into several clusters, with clients in the same cluster sharing the same model, while models can be arbitrarily different across clusters.
Clients jointly learn during training the cluster to which they belong as well as the cluster model. \texttt{FedEM} ~\citep{marfoq2021federated} can  be considered as a soft clustering algorithm  as clients learn personalized models as mixtures of a limited number of component models. 

Multi-Task Learning (MTL) allows for more nuanced relations among clients' models by defining federated MTL as a penalized optimization problem, where the penalization term captures clients' dissimilarity.
Seminal work \citep{smith2017federated,Vanhaesebrouck2017a,pmlr-v108-zantedeschi20a} proposed algorithms able to deal with quite generic penalization terms, at the cost of learning only linear models or linear combinations of pre-trained models.
Other MTL-based algorithms~\citep{hanzely2020federated, hanzely2020lower, dinh2020personalized, dinh2021fedu, li2021ditto, huang2021personalized, li2021ditto} are able to train more general models but consider simpler penalization terms (e.g., the distance to the average model).

An alternative approach is to interpolate a global model and one local model per client~\citep{deng2020adaptive,corinzia2019variational,mansour2020three}. 
\citet{zhang2021personalized} extended this idea by letting each client interpolate the local models of other clients with opportune weights learned during training. Our algorithm, \knnper, also interpolates a global and a local model, but the global model plays a double role as it is also used to provide a useful representation for the local kNN.

Closer to our approach, \texttt{FedRep}~\citep{collins2021exploiting}, \texttt{FedPer}~\citep{Arivazhagan2019FederatedLW} and \pFedGP{} \cite{achituve2021personalized} jointly learn a global latent representation and local models---linear models for \texttt{FedRep} and \texttt{FedPer}, Gaussian processes for \pFedGP---that operate on top of this representation.  
In these algorithms, the progressive refinement of local models affects the shared representation. On the contrary, in \knnper{} only the global model (and then the shared representation) is the object of federated training, and  the shared representation is not influenced by local models, which are learned separately by each client in a second moment. 
Our experiments suggest that \knnper's approach is more efficient. A possible explanation is that jointly learning the shared representation and the local models lead to potentially conflicting and interfering goals.
A similar argument was provided by \citet{li2021ditto} to justify why \texttt{Ditto} replaces, as penalization term, the distance from the average of the local models---as proposed in~\citep{hanzely2020federated, hanzely2020lower, dinh2020personalized}---with the distance from an independently learned global model.
\citet{liang2020think} proposed a someway opposite approach to \texttt{FedRep}, \texttt{FedPer}, and \pFedGP{} by using local representations as input to a global model, but the representations and the global model are still jointly learned.  
An additional advantage of \knnper's clear separation between global and local model training is that, because each client does not share any information about its local model with the server, the risk of leaking private information is reduced. 
In particular, \knnper{} enjoys the same privacy guarantees as \FedAvg{}, and can be easily combined with \emph{differential privacy} techniques \citep{wei2020federated}. 

To the best of our knowledge,  \pFedGP{} and \knnper{} are the first attempts to learn semi-parametric models in a federated setting. \pFedGP{} relies on Gaussian processes and then has higher computational cost than \knnper{} both at training and inference.

\subsection{System Heterogeneity}
Some FL application scenarios envision  clients with highly heterogeneous hardware, like smartphones, IoT devices, edge computing severs, and the cloud.
In this case each client should learn a potentially different model architecture, suited to its capabilities. Such system heterogeneity has been studied much less than statistical heterogeneity.   

Some work~\citep{lin2020ensemble, li2019fedmd, zhu2021datafree, zhang2021fedzkt} proposed to address system heterogeneity by distilling the knowledge from a global teacher to clients' student models with different architectures. While early methods \citep{li2019fedmd, lin2020ensemble} required the access to an extra (unlabeled) public dataset, more recent ones \citep{zhu2021datafree, zhang2021fedzkt} eliminated this requirement. 

Some papers \citep{diao2020heterofl,horvath2021fjord,pilet2021} propose that each client only trains a sub-model  of a global model. The sub-model size is determined by the client's computational capabilities. The approach appears particularly advantageous for convolutional neural networks with clients selecting only a limited subset of channels.

\citet{tan2021fedproto} followed another approach where devices and server communicate prototypes, i.e., average representations for all samples in a given class, instead of communicating model's gradients or parameters, allowing each client to have a different model architecture and input space.

While in this paper we assume that \knnper{} relies on a shared global model, it is possible to replace it with  heterogeneous models adapted to the clients' capabilities and jointly trained following one of the methods listed above. Then, \knnper's  interpolation with a kNN model extends these methods to address not only system heterogeneity, but also statistical heterogeneity. 

To the best of our knowledge, the only existing method that takes into account both system and statistical heterogeneity is \texttt{pFedHN}~\citep{Shamsian2021PersonalizedFL}. \texttt{pFedHN} feeds local clients representations to a global (across clients) hypernetwork, which can output personalized heterogeneous models. Unfortunately, the hypernetwork has a large memory footprint already for  small clients' models (e.g., the hypernetwork in the experiments in~\citep{Shamsian2021PersonalizedFL} has 100 more parameters than the output model): it is not clear if  \texttt{pFedHN} can scale to complex models. 

We observe that  \knnper's  kNN model can itself be adapted to  client's capabilities by tuning the size of the datastore and/or selecting an appropriate approximate kNN algorithm, like FAISS \citep{faiss}, HNSW \citep{malkov2020efficient}, or ProtoNN~\citep{gupta17protonn} for IoT resource-scarce devices, e.g., based on Arduino.

